Compact jets dominate the continuum emission in low-luminosity active galactic nuclei

The disappearance of the accretion disc in low-luminosity active galactic nuclei (LLAGN) leaves behind a faint optical nuclear continuum whose nature has been largely debated, mainly due to serious observational limitations in the IR to UV range. We combine multi-wavelength sub-arcsecond resolution observations -- able to isolate the genuine nuclear continuum -- with nebular lines in the mid-IR, to indirectly probe the shape of the extreme UV continuum. We found that 8 of the nearest prototype LLAGN are compatible with pure compact jet emission (self-absorbed synchrotron plus the associated self-Compton component) over more than ten orders of magnitude in frequency. When compared with typical radio galaxies, the LLAGN continua show two peculiarities: $i)$ a very steep spectral slope in the IR-to-optical/UV range ($-3.7 < \alpha_0 < -1.3$; $F_\nu \propto \nu^{\alpha_0}$); and $ii)$ a very high turnover frequency ($0.2-30\, \rm{THz}$; $1.3\,\rm{mm}-10\,\rm{\mu m}$). These attributes can be explained if the synchrotron continuum is mainly dominated by thermalised particles at the jet base or corona with considerably high temperatures, whereas only a small fraction of the energy ($\sim 20\%$) would be distributed along the high-energy power-law tail of accelerated particles. On the other hand, the nebular gas excitation in LLAGN is in agreement with photo-ionisation from inverse Compton radiation ($\alpha_{\rm x} \sim -0.7$), which would dominate the nuclear continuum shortwards of $\sim 3000$ \r{A}. Our results suggest that the LLAGN continuum can be dominated at all wavelengths by undeveloped jets, powered by a thermalised particle distribution, similar to the behaviour observed in compact jets of quiescent black hole X-ray binaries. This has important implications in the context of galaxy evolution, since LLAGN may represent a major but underestimated source of kinetic feedback in galaxies.

==> tabs/n1052_high.tex <==
%
% MNRAS template returns error if references with '&' in their refcode are not called within {}.
%\hline
%                  & \multicolumn{3}{c}{Model} &  \\
\bf Frequency & \bf F$_\nu$ & \bf Aperture & \bf Telescope/filter & \bf Ref. \\
(Hz) & (Jy) & (radius or beam area) & & \\
%{[Hz]}      & [Jy]    & [radius/beam] &         &           \\
\hline\\[-0.2cm]
$   2.53 \times 10^{19}$ & $(1.5 \pm 0.3) \times 10^{-7}$ &                   & \textit{Swift/BAT}, $14$--$195\, \rm{keV}$ & \citet{2010ApJS..186..378T} \\[0.05cm]
$   1.99 \times 10^{19}$ & $(1.4 \pm 0.8) \times 10^{-7}$ &                   & \textit{Swift/BAT}, $15$--$150\, \rm{keV}$ & {\citet{2010A&A...524A..64C}} \\[0.05cm]
$ 1.6926 \times 10^{19}$ & $1.1 \times 10^{-7}$ &                             & \textit{INTEGRAL}, $40$--$100\, \rm{keV}$  & {\citet{2009A&A...505..417B}} \\[0.05cm]
$  8.463 \times 10^{18}$ & $3.0 \times 10^{-7}$ &                             & \textit{Suzaku}, $10$--$60\, \rm{keV}$     & \citet{2009ApJ...698..528B} \\[0.05cm]
$  8.463 \times 10^{18}$ & $(1.6 \pm 0.2) \times 10^{-7}$ &                   & \textit{Swift/BAT}, $15$--$55\, \rm{keV}$  & \citet{2009ApJ...699..603A} \\[0.05cm]
$  7.254 \times 10^{18}$ & $1.7 \times 10^{-7}$ &                             & \textit{INTEGRAL}, $20$--$40\, \rm{keV}$   & {\citet{2009A&A...505..417B}} \\[0.05cm]
$ 1.4508 \times 10^{18}$ & $2.9^{+0.75}_{-2.44} \times 10^{-7}$ &                & \textit{Chandra}, $2$--$10\, \rm{keV}$     & {\citet{2009A&A...506.1107G}} \\[0.05cm]
$ 1.4508 \times 10^{18}$ & $4.6 \times 10^{-7}$ &                             & \textit{Suzaku}, $2$--$10\, \rm{keV}$      & \citet{2009ApJ...698..528B} \\[0.05cm]
$ 1.1046 \times 10^{15}$ & $(8.1 \pm 0.3) \times 10^{-6}$ & $0\farcs15$       & \textit{HST}/ACS-HRC, F250W    & \citet{jafo2019}     \\[0.05cm]
$ 8.9206 \times 10^{14}$ & $(1.48 \pm 0.03) \times 10^{-5}$ & $0\farcs15$     & \textit{HST}/ACS-HRC, F330W    & \citet{jafo2019}     \\[0.05cm]
$ 5.5006 \times 10^{14}$ & $(3.4 \pm 0.1) \times 10^{-5}$ & $0\farcs15$       & \textit{HST}/WFPC1, F555W      & \citet{jafo2019}     \\[0.05cm]
$ 2.3715 \times 10^{14}$ & $(6.3 \pm 0.1) \times 10^{-4}$ & $0\farcs26$       & VLT/NaCo, \textit{J} band      & \citet{jafo2019}     \\[0.05cm]
$  1.868 \times 10^{14}$ & $(8.0 \pm 0.3) \times 10^{-4}$ & $0\farcs15$       & \textit{HST}/NIC2, F160W       & \citet{jafo2019}     \\[0.05cm]
$ 1.3761 \times 10^{14}$ & $(1.19 \pm 0.02) \times 10^{-3}$ & $0\farcs15$     & VLT/NaCo, \textit{Ks} band     & \citet{jafo2019}     \\[0.05cm]
$ 7.8947 \times 10^{13}$ & $(7.17 \pm 0.03) \times 10^{-3}$ & $0\farcs15$     & VLT/NaCo, \textit{L'} band     & \citet{jafo2019}     \\[0.05cm]
$   3.86 \times 10^{13}$ & $(58.8 \pm 9.4) \times 10^{-3}$ & $0\farcs52 \times 0\farcs39$      & VLT/VISIR, J7.9          & \citet{asmus2014} \\[0.05cm]
$   3.49 \times 10^{13}$ & $(62.4 \pm 14.4) \times 10^{-3}$ & $0\farcs45 \times 0\farcs39$      & VLT/VISIR, PAH1          & \citet{asmus2014} \\[0.05cm]
$   3.49 \times 10^{13}$ & $(58 \pm 14) \times 10^{-3}$   & $0\farcs45 \times 0\farcs40$      & VLT/VISIR, PAH1          & \citet{jafo2019} \\[0.05cm]
$  3.446 \times 10^{13}$ & $(63 \pm 6) \times 10^{-3}$    &   $0\farcs5$                      & GTC/CanariCam, Si2                             & \citet{jafo2019} \\[0.03cm]
$   3.43 \times 10^{13}$ & $(63.6 \pm 1.6) \times 10^{-3}$   & $0\farcs75 \times 0\farcs62$      & Gemini/T-ReCS, Si2       & \citet{asmus2014} \\[0.05cm]
$   3.05 \times 10^{13}$ & $(114.7 \pm 22.9) \times 10^{-3}$ & $0\farcs39 \times 0\farcs35$     & VLT/VISIR, B9.7          & \citet{asmus2014} \\[0.05cm]
$   2.81 \times 10^{13}$ & $(133.7 \pm 22.8) \times 10^{-3}$ & $0\farcs43 \times 0\farcs37$     & VLT/VISIR, B10.7         & \citet{asmus2014} \\[0.05cm]
$    2.6 \times 10^{13}$ & $(154.1 \pm 13.2) \times 10^{-3}$ & $0\farcs44 \times 0\farcs40$     & VLT/VISIR, B11.7         & \citet{asmus2014} \\[0.05cm]
$  2.584 \times 10^{13}$ & $(123 \pm 12) \times 10^{-3}$ & $0\farcs5$                          & GTC/CanariCam, Si5                             & \citet{jafo2019} \\[0.03cm]
$   2.52 \times 10^{13}$ & $(133.9 \pm 4.2) \times 10^{-3}$ & $0\farcs40 \times 0\farcs36$     & VLT/VISIR, PAH2\_2       & \citet{asmus2014} \\[0.05cm]
$   2.52 \times 10^{13}$ & $(133 \pm 4) \times 10^{-3}$   & $0\farcs40 \times 0\farcs40$     & VLT/VISIR, PAH2\_2       & \citet{jafo2019} \\[0.05cm]
$    2.4 \times 10^{13}$ & $(181.2 \pm 19.8) \times 10^{-3}$ & $0\farcs51 \times 0\farcs42$     & VLT/VISIR, B12.4         & \citet{asmus2014} \\[0.05cm]
$   1.64 \times 10^{13}$ & $(355.7 \pm 9.1) \times 10^{-3}$ & $0\farcs55 \times 0\farcs52$     & Gemini/T-ReCS, Qa        & \citet{asmus2014} \\[0.05cm]
$    1.6 \times 10^{13}$ & $(339.0 \pm 33.8) \times 10^{-3}$ & $0\farcs50 \times 0\farcs49$     & VLT/VISIR, Q2            & \citet{asmus2014} \\[0.05cm]
$  4.778 \times 10^{11}$ & $(201 \pm 2) \times 10^{-3}$      & $0\farcs12 \times 0\farcs10$     & ALMA, $478\, \rm{GHz}$   & \citet{jafo2019} \\[0.05cm]
$  4.657 \times 10^{11}$ & $(207 \pm 1) \times 10^{-3}$      & $0\farcs12 \times 0\farcs10$     & ALMA, $466\, \rm{GHz}$   & \citet{jafo2019} \\[0.05cm]
$  4.315 \times 10^{11}$ & $(273 \pm 1) \times 10^{-3}$      & $0\farcs13 \times 0\farcs12$     & ALMA, $432\, \rm{GHz}$   & \citet{jafo2019} \\[0.05cm]
$  4.194 \times 10^{11}$ & $(283 \pm 1) \times 10^{-3}$      & $0\farcs14 \times 0\farcs12$     & ALMA, $419\, \rm{GHz}$   & \citet{jafo2019} \\[0.05cm]
$  3.528 \times 10^{11}$ & $(283.1 \pm 1.1) \times 10^{-3}$  & $0\farcs20 \times 0\farcs15$     & ALMA, $353\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$  3.408 \times 10^{11}$ & $(299.3 \pm 1.1) \times 10^{-3}$  & $0\farcs20 \times 0\farcs15$     & ALMA, $341\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$  2.294 \times 10^{11}$ & $(457 \pm 4) \times 10^{-3}$      & $0\farcs3 \times 0\farcs2$       & ALMA, $229\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$  2.141 \times 10^{11}$ & $(495 \pm 3) \times 10^{-3}$      & $0\farcs3 \times 0\farcs2$       & ALMA, $214\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$  1.080 \times 10^{11}$ & $(750 \pm 7) \times 10^{-3}$      & $0\farcs7 \times 0\farcs6$       & ALMA, $108\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$    8.9 \times 10^{10}$ & $0.561^*$           & $1.44 \times 0.90\, \rm{mas^2}$ & KVN, $89\, \rm{GHz}$                    & \citet{2016ApJ...830L...3S} \\[0.05cm]
$    8.6 \times 10^{10}$ & $0.62 \pm 0.09^*$   & $0.407 \times 0.075\, \rm{mas^2}$ & GMVA, $86\, \rm{GHz}$  & {\citet{2016A&A...593A..47B}} \\[0.05cm]
$    4.3 \times 10^{10}$ & $0.49$--$1.64$            & $1.11  \times 0.21\, \rm{mas^2}$  & VLBI, $43\, \rm{GHz}$, min--max 2005-2009    & {\citet{2019A&A...623A..27B}} \\[0.05cm]
%$    4.3 \times 10^{10}$ & $0.49$            & $0.40  \times 0.16\, \rm{mas^2}$  & VLBI, $43\, \rm{GHz}$, min 2005-2009    & \citet{2019A&A...623A..27B} \\[0.05cm]
%$    4.3 \times 10^{10}$ & $0.67^*$          & $0.45 \times 0.16\, \rm{mas^2}$  & VLBI, $43\, \rm{GHz}$                    & {\citet{2004A&A...426..481K}} \\[0.05cm]
$   2.21 \times 10^{10}$ & $2.46 \pm 0.02$   & $0\farcs09 \times 0\farcs07$       & JVLA, $22\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$    2.2 \times 10^{10}$ & $0.50$--$2.26$            & $0.96  \times 0.37\, \rm{mas^2}$  & VLBI, $22\, \rm{GHz}$, min--max 2005-2009    & {\citet{2019A&A...623A..27B}} \\[0.05cm]
%$    2.2 \times 10^{10}$ & $0.50$            & $0.96  \times 0.34\, \rm{mas^2}$  & VLBI, $22\, \rm{GHz}$, min 2005-2009    & \citet{2019A&A...623A..27B} \\[0.05cm]
%$    2.2 \times 10^{10}$ & $1.51^*$          & $0.86  \times 0.32\, \rm{mas^2}$  & VLBI, $22\, \rm{GHz}$                   & {\citet{2004A&A...426..481K}} \\[0.05cm]
$ 1.5364 \times 10^{10}$ & $1.99 \pm 0.04^*$ & $1.03  \times 0.40\, \rm{mas^2}$  & VLBA, $15\, \rm{GHz}$ & \citet{2001PASJ...53..169K} \\[0.05cm]
$   1.49 \times 10^{10}$ & $1.0 \pm 0.1$     & $0\farcs1 \times 0\farcs09$       & JVLA, $15\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$    8.4 \times 10^{9}$ & $2.91 \pm 0.03$     & $0\farcs3 \times 0\farcs2$       & JVLA, $8.4\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$    8.4 \times 10^{9}$ & $2.39^*$           & $1.98  \times 0.81\, \rm{mas^2}$  & VLBI, $8.4\, \rm{GHz}$                  & {\citet{2004A&A...426..481K}} \\[0.05cm]
$    6.2 \times 10^{9}$ & $1.295 \pm 0.001$     & $0\farcs4 \times 0\farcs3$     & JVLA, $6.2\, \rm{GHz}$   & \citet{pasetto2019} \\[0.05cm]
$    5.0 \times 10^{9}$ & $2.41^*$           & $3.3   \times 1.31\, \rm{mas^2}$  & VLBI, $5\, \rm{GHz}$                    & {\citet{2004A&A...426..481K}} \\[0.05cm]
$   2.32 \times 10^{9}$ & $1.51^*$           & $9.0   \times 3.8\, \rm{mas^2}$   & VLBA, $2.3\, \rm{GHz}$                  & \citet{1997ApJS..111...95F} \\[0.05cm]
$ 1.6710 \times 10^{9}$ & $0.62 \pm 0.06$  & $3.40\, \rm{mas}$               & VLBI, $1.7\, \rm{GHz}$                      & \citet{1979ApJ...233L.105S} \\[0.05cm]
$   3.27 \times 10^{8}$ & $0.30 \pm 0.15$   & $0\farcs1$                        & Ooty Radio Telescope, $327\, \rm{MHz}$    & \citet{1984IAUS..110..261B} \\[0.05cm]
\hline


==> tabs/n1052_low.tex <==
%
% MNRAS template returns error if references with '&' in their refcode are not called within {}.
%
\bf Frequency & \bf F$_\nu$ & \bf Aperture & \bf Telescope/filter & \bf Ref. \\
(Hz) & (Jy) & (radius or beam area) & & \\
\hline\\[-0.2cm]
$   1.95 \times 10^{15}$ &$ (7.7 \pm 0.6) \times 10^{-5}$ & $4\farcs21$ & \textit{GALEX} FUV                             & \citet{marino2011} \\[0.03cm]
$   1.29 \times 10^{15}$ &$ (1.47 \pm 0.06) \times 10^{-4}$ & $4\farcs21$ & \textit{GALEX} NUV                             & \citet{marino2011} \\[0.03cm]
$   2.38 \times 10^{14}$ &$ (2.6 \pm 0.3) \times 10^{-2}$ &       $2''$ & InfraRed Telescope Facility (IRTF), \textit{J} band & \citet{1982ApJ...263..624B} \\[0.03cm]
$   1.87 \times 10^{14}$ &$ (3.5 \pm 0.3) \times 10^{-2}$ &       $2''$ & IRTF, \textit{H} band                          & \citet{1982ApJ...263..624B} \\[0.03cm] 
%$ 1.3761 \times 10^{14}$ & $ 1.27 \times 10^{-2}$  & $0\farcs75$ & VLT/NaCo, \textit{Ks} band                     & \citet{jafo2019}     \\[0.03cm]
$   1.35 \times 10^{14}$ &$ (3.2 \pm 0.3) \times 10^{-2}$ &       $2''$ & IRTF, \textit{K} band                          & \citet{1982ApJ...263..624B} \\[0.03cm]
$   8.47 \times 10^{13}$ &$ (2.8 \pm 0.3) \times 10^{-2}$ &       $2''$ & IRTF, \textit{L} band                          & \citet{1982ApJ...263..624B} \\[0.03cm]
$ 8.3333 \times 10^{13}$ &$ 4.0 \times 10^{-2}$ &  $2\farcs4$ & \textit{Spitzer} $3.6\, \rm{\micron}$          & \citet{jafo2019}                   \\[0.03cm] 
$ 6.6667 \times 10^{13}$ &$ 3.7 \times 10^{-2}$ &  $2\farcs4$ & \textit{Spitzer} $4.5\, \rm{\micron}$          & \citet{jafo2019}                   \\[0.03cm] 
$   6.25 \times 10^{13}$ &$ (3.0 \pm 0.4) \times 10^{-2}$ &       $4''$ & IRTF, \textit{M} band                          & \citet{1982ApJ...263..624B} \\[0.03cm]
$ 5.1724 \times 10^{13}$ &$ 4.7 \times 10^{-2}$ &  $2\farcs4$ & \textit{Spitzer} $5.8\, \rm{\micron}$          & \citet{jafo2019}                                       \\[0.03cm] 
$   3.75 \times 10^{13}$ &$ 6.9 \times 10^{-2}$ &  $2\farcs4$ & \textit{Spitzer} $8.0\, \rm{\micron}$          & \citet{jafo2019}                                       \\[0.03cm] 
$ 3.3333 \times 10^{13}$ & $(15 \pm 3) \times 10^{-2}$ & $\sim 5\farcs5$ & \textit{Akari}/IRC $9\, \rm{\micron}$, Point Source Catalogue & NASA/IPAC Infrared Science Archive \\[0.03cm] 
$   2.83 \times 10^{13}$ & $(11.1 \pm 1.6) \times 10^{-2}$ & $4''$ & IRTF, \textit{N} band                          & \citet{1982ApJ...263..624B}  \\[0.03cm] 
$  2.595 \times 10^{13}$ & $(15.7 \pm 0.2) \times 10^{-2}$ &  $7\farcs4$ & \textit{WISE} W3, AllWISE Source Catalog       & NASA/IPAC Infrared Science Archive             \\[0.03cm] 
$    2.5 \times 10^{13}$ & $(13.8 \pm 0.2) \times 10^{-2}$ & $\sim 30''$ & \textit{IRAS} $12\, \rm{\micron}$, IRS enhanced products & NASA/IPAC Infrared Science Archive \\[0.03cm]
$ 1.6667 \times 10^{13}$ & $(38 \pm 0.02) \times 10^{-2}$ & $\sim 5\farcs7$ & \textit{Akari}/IRC $18\, \rm{\micron}$, Point Source Catalogue & NASA/IPAC Infrared Science Archive \\[0.03cm]
$   1.47 \times 10^{13}$ & $(46 \pm 7) \times 10^{-2}$ &   $4''$ & IRTF, \textit{Q} band                          & \citet{1982ApJ...263..624B}  \\[0.03cm]
$ 1.3582 \times 10^{13}$ & $(44.3 \pm 0.9) \times 10^{-2}$ & $\sim 12''$ & \textit{WISE} W4, AllWISE Source Catalog       & NASA/IPAC Infrared Science Archive             \\[0.03cm] 
$   1.27 \times 10^{13}$ & $(41.4 \pm 0.8) \times 10^{-2}$ &     & \textit{Spitzer}/MIPS $24\, \rm{\micron}$, IRS enhanced products & NASA/IPAC Infrared Science Archive \\[0.03cm]
$    1.2 \times 10^{13}$ & $(42.2 \pm 0.7) \times 10^{-2}$ & $\sim 30''$ & \textit{IRAS} $25\, \rm{\micron}$, IRS enhanced products & NASA/IPAC Infrared Science Archive \\[0.03cm]
$      5 \times 10^{12}$ &                 $0.94$ & $\sim 60''$ & \textit{IRAS} $60\, \rm{\micron}$, Point Source Catalog v2.1 & NASA/IPAC Infrared Science Archive \\[0.03cm]
$ 4.6154 \times 10^{12}$ &                $0.84$ & $\sim  50''$ & \textit{Akari}/FIS $65\, \rm{\micron}$, Bright Source Catalogue & NASA/IPAC Infrared Science Archive             \\[0.03cm]
$ 4.2827 \times 10^{12}$ & $(73.7 \pm 1.5) \times 10^{-2}$ & $6\farcs25 \times 5\farcs35$ & \textit{Herschel}/PACS $70\, \rm{\micron}$, Point Source Catalog & NASA/IPAC Infrared Science Archive \\[0.03cm]
$ 3.3333 \times 10^{12}$ & $(79 \pm 4) \times 10^{-2}$ & $\sim  50''$ & \textit{Akari}/FIS $90\, \rm{\micron}$, Bright Source Catalogue & NASA/IPAC Infrared Science Archive             \\[0.03cm]
$      3 \times 10^{12}$ &                 $1.22$ &  $\sim 2'$ & \textit{IRAS} $100\, \rm{\micron}$, Point Source Catalog v2.1 & NASA/IPAC Infrared Science Archive \\[0.03cm]
$ 2.1429 \times 10^{12}$ &          $1.3 \pm 0.4$ & $\sim  90''$ & \textit{Akari}/FIS $140\, \rm{\micron}$, Bright Source Catalogue & NASA/IPAC Infrared Science Archive             \\[0.03cm]
$  1.875 \times 10^{12}$ &                  $0.9$ & $\sim  90''$ & \textit{Akari}/FIS $160\, \rm{\micron}$, Bright Source Catalogue & NASA/IPAC Infrared Science Archive             \\[0.03cm]
$ 1.8737 \times 10^{12}$ & $0.65 \pm 0.18$ & $17\farcs88 \times 11\farcs52$ & \textit{Herschel}/PACS $160\, \rm{\micron}$, Point Source Catalog & NASA/IPAC Infrared Science Archive \\[0.03cm]
$  6.667 \times 10^{11}$ &      $0.941 \pm 0.785$ &      $15''$ & JCMT $0.45\, \rm{mm}$                          & \citet{1991AJ....101.1609K} \\[0.03cm] 
$   3.75 \times 10^{11}$ &      $0.412 \pm 0.039$ &      $17''$ & JCMT $0.8\, \rm{mm}$                           & \citet{1991AJ....101.1609K} \\[0.03cm]
$ 2.7273 \times 10^{11}$ &      $0.511 \pm 0.019$ & $18\farcs5$ & JCMT $1.1\, \rm{mm}$                           & \citet{1991AJ....101.1609K} \\[0.03cm]
$ 2.3077 \times 10^{11}$ &      $0.563 \pm 0.028$ & $19\farcs5$ & JCMT $1.3\, \rm{mm}$                           & \citet{1991AJ....101.1609K} \\[0.03cm]
$    1.5 \times 10^{11}$ &      $1.036 \pm 0.083$ & $27\farcs5$ & JCMT $2.0\, \rm{mm}$                           & \citet{1991AJ....101.1609K} \\[0.03cm]
$   8.96 \times 10^{10}$ &          $2.0 \pm 0.5$ & $\sim 60''$ & NRAO 11\,m telescope $89.6\, \rm{GHz}$, event A 05/1973   & \citet{1983ApJ...267L..11H} \\[0.03cm]
$   8.96 \times 10^{10}$ &          $1.2 \pm 0.5$ & $\sim 60''$ & NRAO 11\,m telescope $89.6\, \rm{GHz}$, event B 02/1980   & \citet{1983ApJ...267L..11H} \\[0.03cm]
$   8.57 \times 10^{10}$ &        $0.91 \pm 0.24$ & $\sim 65''$ & NRAO 11\,m telescope $3.5\, \rm{mm}$, average 1968-1973   & \citet{1975ApJ...196..347H} \\[0.03cm]
$   8.57 \times 10^{10}$ &        $2.21 \pm 0.52$ & $\sim 65''$ & NRAO 11\,m telescope $3.5\, \rm{mm}$, 07/1973             & \citet{1975ApJ...196..347H} \\[0.03cm]
$   3.16 \times 10^{10}$ &        $1.52 \pm 0.24$ &   $\sim 3'$ & NRAO 11\,m telescope $9.5\, \rm{mm}$, average 1968-1973   & \citet{1975ApJ...196..347H} \\[0.03cm]
$   3.16 \times 10^{10}$ &        $2.86 \pm 0.24$ &   $\sim 3'$ & NRAO 11\,m telescope $9.5\, \rm{mm}$, 07/1973             & \citet{1975ApJ...196..347H} \\[0.03cm]
$   3.14 \times 10^{10}$ &          $2.9 \pm 0.2$ &   $\sim 3'$ & NRAO 11\,m telescope $31.4\, \rm{GHz}$, event A 05/1973   & \citet{1983ApJ...267L..11H} \\[0.03cm]
$   3.14 \times 10^{10}$ &          $1.7 \pm 0.2$ &   $\sim 3'$ & NRAO 11\,m telescope $31.4\, \rm{GHz}$, event B 02/1980   & \citet{1983ApJ...267L..11H} \\[0.03cm]
$    2.2 \times 10^{10}$ &       $1.62 \pm 0.162$ &       $7''$ & ATCA $22\, \rm{GHz}$                                      & {\citet{2006A&A...445..465R}} \\[0.03cm]
$   1.55 \times 10^{10}$ &          $2.0 \pm 0.1$ &   $\sim 6'$ & NRAO 11\,m telescope $15.5\, \rm{GHz}$, event A 05/1973   & \citet{1983ApJ...267L..11H} \\[0.03cm]
$   1.55 \times 10^{10}$ &          $1.8 \pm 0.1$ &   $\sim 6'$ & NRAO 11\,m telescope $15.5\, \rm{GHz}$, event B 02/1980   & \citet{1983ApJ...267L..11H} \\[0.03cm]
 $    8.6 \times 10^{9}$ &                 $2.63$ &       $1''$ & ATCA $8.6\, \rm{GHz}$                          & \citet{2003PASJ...55..351T} \\[0.03cm]
 $    4.8 \times 10^{9}$ &                 $2.47$ &       $2''$ & ATCA $4.8\, \rm{GHz}$                          & \citet{2003PASJ...55..351T} \\[0.03cm]
 $    2.5 \times 10^{9}$ &                 $1.46$ &  $4\farcs5$ & ATCA $2.5\, \rm{GHz}$                          & \citet{2003PASJ...55..351T} \\[0.03cm]
 $ 1.6649 \times 10^{9}$ & $(83.1 \pm 1.7) \times 10^{-2}$ & $1''$ & VLA $1.66\, \rm{GHz}$                          & \citet{1984ApJ...284..531W} \\[0.03cm]
 $ 1.3851 \times 10^{9}$ & $(73.5 \pm 1.5) \times 10^{-2}$ & $1''$ & VLA $1.39\, \rm{GHz}$                          & \citet{1984ApJ...284..531W} \\[0.03cm]
 $   4.08 \times 10^{8}$ &        $0.84 \pm 0.04$ &             & Molonglo Radio Telescope $408\, \rm{MHz}$      & \citet{1981MNRAS.194..693L} \\[0.03cm]
 $   3.65 \times 10^{8}$ &                 $0.64$ &             & Texas Interferometer $365\, \rm{MHz}$          & \citet{1996AJ....111.1945D} \\[0.03cm]
 $   7.38 \times 10^{7}$ &        $0.85 \pm 0.13$ & $\sim 80''$ & VLA $74\, \rm{MHz}$                            & \citet{cohen2007} \\
\hline

